Enhanced Prediction of CO2 Solubility under Geological Conditions for CCUS via Improved Pitzer Parameters and Physics-Informed Machine Learning

The solubility of CO2 in formation brines plays a critical role in the efficiency of carbon capture and storage (CCS) operations. It is strongly influenced by pressure, temperature, and brine composition. Various experimental studies and modeling approaches have been developed to estimate CO2 solubility under wide ranges of pressure, temperature, and salinities. This work makes three key contributions. First, we present an extensive literature review of experimental, theoretical, and simulation-based approaches for measuring and predicting CO2 solubility across a wide range of conditions and also a discussion of how the different parameters affect solubility. Second, we introduce an improved set of temperature-dependent Pitzer interaction parameters, yielding up to a 76% reduction in average absolute deviation compared to conventional values in the geochemical simulation software PHREEQC. Third, we develop a physics-informed machine learning model that integrates thermodynamic intuition with data-driven learning, achieving a 14% reduction in prediction error over the state-of-the-art and up to 40% improvement at high salinities. Together, these advances provide a robust and accurate framework for predicting CO2 solubility, supporting more reliable CCS design and deployment.

==> sections/trends_water_chemistry.tex <==
\subsection{Effect of water chemistry}
Solubility is highly affected by water composition, characterized by the concentration and types of aqueous species. While the effect of pressure and temperature is relatively straightforward, water chemistry effect is a bit more nuanced. Here we will discuss the effect of different ions or aqueous species that are common in natural formation brines, how they affect solubility, and to what extent.

%\subsubsection{The carbonate system}

In \HtwoO--\COtwo system, \COtwo first dissolves into water as an aqueous species (Equation \ref{eq:co2_gas_to_aqueous}) to form aqueous \COtwo. Dissolved or aqueous \COtwo then reacts with water to form carbonic acid, \carbonic (Equation \ref{eq:carbonic_acid_formation}). The formed \carbonic then dissociates into a proton, \proton, and a bicarbonate ion, \bicarbonate (Equation \ref{eq:bicarbonate_formation}). Finally, \bicarbonate dissociates further into \proton and a carbonate ion, \carbonate (Equation \ref{eq:carbonate_formation}). Figure \ref{fig:carbonate} shows the fraction of different carbon species as a function of pH. 

\begin{align}
    CO_2(g) &\rightleftharpoons CO_2(aq) \label{eq:co2_gas_to_aqueous} \\
    CO_2(aq) + H_2O(l) &\rightleftharpoons H_2CO_3(aq) \label{eq:carbonic_acid_formation} \\
    H_2CO_3(aq) &\rightleftharpoons HCO_3^-(aq) + H^+(aq) \label{eq:bicarbonate_formation} \\
    HCO_3^-(aq) &\rightleftharpoons CO_3^{2-}(aq) + H^+(aq) \label{eq:carbonate_formation}
\end{align}



\begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/carbonate.png}
    \caption{Distribution of carbon species in water as a function of pH (at $T=25\degree C$)}
    \label{fig:carbonate}
\end{figure}

At typical storage conditions (pH \textless 4.0), most of the dissolved \COtwo exists as aqueous \COtwo \citep{DeSilva2015,Gilbert2016}. Neutral species such as \COtwoaq are subject to \textit{salting-out} by ions dissolved in the formation water. Salting-out refers ot the reduction in solubility of \COtwo (and other substances) with the addition of inorganic salts to the solution. 
%This can be explained by the fact that when salts are dissolved, more ions are solvated or hydrated, more water molecules are trapped in the ions' hydration shell (Figure \ref{fig:hydration_shell}) and less water molecules are available for dissolving other substances \citep{Liu2011}.



Numerous works assume the ionic strength of the solution as the main factor influencing the salting-out effect \citep{Gilbert2016, Zhao2015, Portier2005}. Molal ionic strength, $I$, is given by Equation \ref{eq:ionic_strength}. $b_i$ is the molality of ion $i$ and $z_i$ is its charge.

\begin{equation}
    I = \frac{1}{2} \sum_i^n b_iz_i^2
    \label{eq:ionic_strength}
\end{equation}

This assumption allows for simpler experimental studies, as it is enough to match the ionic strength of the brine in your target formation with simpler brines (e.g., NaCl) and assume the salting-out effect will be  the same \citep{Zhao2015c}. While this can be a good approximation, ionic strength is not enough as different salts, and consequently different ions, contribute differently to salting-out.

Figure \ref{fig:solubility_1_3_molal} illustrates the variation of solubility in NaCl, KCl, \CaCltwo, \MgCltwo, and \NaSOfour solutions, at concentrations of 1, 2, and 3 molal, with solubility in pure water as a reference. 



\begin{figure}[H]
    \includegraphics[width=\linewidth]{figures/solubility_at_1_3_molality.png}
    \caption{\COtwo solubility in different solutions with concentrations from 1m to 3m at 323.15K}
    \label{fig:solubility_1_3_molal}
\end{figure}

Lines are simulation data obtained from PHREEQC using \texttt{pitzer.dat}, while data points are experimental measurements from \citet{Wang2019, Zhao2015b, dosSantos2020, dosSantos2021, LaraCruz2020, Messabeb2017}. At the same molality, NaCl and KCl solutions have the same ionic strength. This is also true for  \MgCltwo, \CaCltwo, and \NaSOfour solutions at the same molality. It is clear that at the same ionic strength, the salting-out effect is different for different solutions. Salting-out effect of different salts at the same concentration (not strictly same ionic strength) increases in the following order: KCl \textless NaCl \textless \MgCltwo \textless \CaCltwo \textless \NaSOfour. It is therefore a complex phenomneon that results from different interactions, such as the hydration of ions \citep{Gorgenyi2006} and the formation of ion pairs \citep{Gilbert2016}.

When salts dissolve in water, a shell of water molecules surrounds the ions, forming a \textit{solvation} or \textit{hydration shell} (Figure \ref{fig:hydration_shell}). The presence of ions in a solution restricts the movement of water molecules and leaves less water to dissolve other species such as \COtwo. The hydration shell structure is a function of the charge of the ion and its sign, and the ionic radius.

Hydration of cations and anions are different, even when they are characterized by same charge and similar ionic radii \citep{Yang2011}.  \sodium has a smaller atomic radius than potassium while having the same charge, resulting in a higher charge density and a greater ordering of water molecules \citep{Hribar2002}. \calcium has a slightly weaker hydration compared to \magnesium due to the smaller ionic radii of the latter \citep{Friesen2019} (72pm for \magnesium and 106pm for \calcium \citep{Shannon1976})

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/hydration_shell.png}
    \caption{Schematic of hydration shells around ions.}
    \label{fig:hydration_shell}
\end{figure}

\textit{Electrostricted water}, which refers to the concentraiton of water molecules needed to hydrate ions in a solution, can be a better predictor of the salting-out of \COtwo than ionic strength. This approach was suggested by \citet{Gilbert2016}, and the formula to determine the concentration of electrostricted water, $h_a$, is given by Equation \ref{eqn:electrostricted}, where $C_i$ is the concentration of an ion $i$, $n_i$ is the stoichiometric coefficient, and $h_{comp}$ is the hydration number. 

\begin{equation}
    h_a = \sum C_in_ih_{comp}
    \label{eqn:electrostricted}
\end{equation}

Figure \ref{fig:electrostriction} shows change in solubility as a function of $h_a$, with experimental data from \citep{dosSantos2020,dosSantos2021,Kamps2007,Koschel2006,LaraCruz2020,Liu2011,Messabeb2017,Rumpf1993,Tong2013,Wang2019,Yan2011,Zhao2015,Zhao2015b,Zhao2015c, Bermejo2005}. The fitted ordinary least squares lines have high coefficients of determination ($R^2 \geq 0.89$) indicating that the concentraiton of electrostricted water molecules is a strong predictor of salting-out. Despite the good agreement with experimental data, this approach is not perfect because it assumes that ion hydration is additive. Studies showed that ion hydration is cooperative and non-additive rather than additive where \citep{Tielrooij2010}. The determination of hydraiton numbers is also tricky and they are inconsistent among studies \citep{Marcus2014}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/electrostriction.png}
    \caption{Isothermal (top) and isobaric (bottom) solubilities of \COtwo as a function of molality of electrostricted water.}
    \label{fig:electrostriction}
\end{figure}

Ion pairs and clusters start to form even at lower concentrations and increase with increasing ionic strength \citep{Chen2015, Ohtaki1993, Marcus2014}. Ion pairs can be either contact ion pairs (CIPs), solvent-shared ion pairs (SIPs), or double solvent-separated ion pairs (2SIPs) \citep{Friesen2019}. 
The formation of ion pairs can also influence the salting-out effect. These ion pairs can be neutral such as NaCl\textsuperscript{0}, or have a lower charge density such as  MgCl\textsuperscript{+}, CaCl\textsuperscript{+}, and NaSO\textsubscript{4}\textsuperscript{-}. 























%\begin{table}[H]
%    \caption{Hydration numbers of different ions}
%    \centering
%\begin{tabular}{p{30mm}cc}
%    \hline
%    \textbf{Brine}   &   \textbf{Hydration} & \textbf{Ref.} \\
%    \hline
%    \multicolumn{3}{c}{\textbf{Isothermic system (T=323.15K)}}\\
    

%    \hline

    
%    NaCl = 1.06 \newline \MgCltwo (0.05), KCl (0.02), \CaCltwo (0.14); Na\textsubscript{2}SO\textsubscript{4}&   9.464    &  \citet{Zhao2015c}\\
%    HCO\textsubscript{3}\textsuperscript{-} &   1.7    &  \\
%    \hline
%\end{tabular}
%\end{table}


%Aqueous species affect solubility of \COtwo in water by increasing the ionic strength of the solution, and thereby increasing the concentration of electrostricted water, which means the solvent (i.e. water) will have less free water molecules to interact with \COtwo. Since different salts introduce different ions with different electrical and physical properties, different salts, therefore ions, will affect solubility differently. The hydration number of an ion refers to the number of water molecules surrounding the ion and forming the hydration shell, and it is a function of the ion's charge and atomic radius. Ionic strength and electrostricted water concentration should be therefore highly correlated, and both should also correlate to the extent of \COtwo solubility (a linear correlation for a given pressure and temperature).


%From Figure \ref{fig:solubility_1_3_molal} we can see that salinity or concentration of ionic species is not clearly indicative of the extent of solubility in water. Different ions affect solubility to different extents. This can be attributed mainly to ion's ionic radius and charge, which directly influences the hydration shell around that ion, and eventually the concentration of electrostricted water. We calculated the molality of electrostricted water, $H$, using Equation \ref{eqn:electrostricted}:



%------------------------------------------------------------


%\citep{Yang2011}: Simulations performed on these systems all indicate that the hydration of cations are different from that of anions, even when other properties (such as the radius) of the ions are the same. In the hydration of anions, water molecules can approach closer to the ion, presumably as a result of the positive charge carried by the hydrogen being closer to the periphery of the water molecule and allows for stronger electrostatic interaction between the anions and water. . Since the current simulations were performed with very simple fixed point charge models, the origin of the observed different behaviors of charged particles with all identical properties except for the charge sign must lie in the charge asymmetry of the water model used. For example, in the SPC/E model, the negative charge is closer to the center of the molecule than the two positive partial charges carried at the two hydrogen atoms. As a result, although each of the positive charges have only half of the magnitude of the negative one, anions can approach closer to the positive charges of water than the cations do to the negative charge located at the oxygen atom.



%\citep{Ohtaki1993} In concentrated electrolyte solutions, ion pairs and complexes are often formed, which still include water molecules in the first coordination shell of the central ions. Smaller ionic radius results in larger hydration. Water is a moderate donor and a rather strong acceptor solvent, and thus, water is expected to solvate anions more strongly than cations. However, hydration of anions is usually much weaker than that of cations, except for limited cases such as OH" and F-, because most anions have much larger ionic radii than cations. In fact, the hydration enthalpy of F~ is more negative than that of Na+ which has a similar or even smaller ionic radius than F-.203 Therefore, information on the hydration structure of anions is not very conclusive compared with that of cations in spite of fairly large number of measurements have been ca




%------------------------------------------------------------

%\citet{Portier2005} used a salting coefficient $\sigma_{CO_2}$ which is multiplied by the ionic strengt of the solution to determine the activity coefficient of \COtwo. However, the authors acknowledge the limitation of this approach of matching ionic strengths to NaCl. \citep{Zhao2015}



%This can be attributed to K\textsuperscript{+} having a lower hydration number than Na\textsuperscript{+}. Mg\textsuperscript{2+} and Ca\textsuperscript{2+} have the same hydration number, and their effect is almost identical. Simulation shows an identical solubility \MgCltwo and \CaCltwo. This discrepancy between simulation and experimental results can be attributed to the fact that both Mg\textsuperscript{2+}--\COtwo and Cl\textsuperscript{2+}--\COtwo have the same Pitzer binary interaction parameter $\lambda_{ij}=0.183$. 


%Salting-out effect of \CaCltwo is higher than that of NaCl. Although it is hard to directly to compare them directly, since \CaCltwo contributes double the number of anions,  however, calcium and sodium have a very similar atomic radii, while the calcium cation is doubly-charged and therefore has a much higher hydration number and a higher salting-out effect. Other studies concluded that their salting-out effect is similar, however, the conclusion was based on experimental measurements using an equal wt\%, and given that the molar mass of \CaCltwo is double that of NaCl, which can significantly skew the results.


% \begin{table}[H]
%     \caption{Hydration numbers of different ions}
%     \centering
% \begin{tabular}{cc}
%     \hline
%     Ion &   Hydration number\\
%     \hline
%     Na\textsuperscript{+}   &   3.3 \\
%     Cl\textsuperscript{-}   &   2.7 \\
%     K\textsuperscript{+}    &   2.3 \\
%     Mg\textsuperscript{2+}  &   8.9 \\
%     Ca\textsuperscript{2+}  &   8.9 \\
%     SO\textsubscript{4}\textsuperscript{2-} &   10.4    \\
%     HCO\textsubscript{3}\textsuperscript{-} &   1.7     \\
%     \hline
% \end{tabular}
% \end{table}
